White Paper on Software Infrastructure for Advanced Nuclear Physics Computing

This White Paper documents the discussion and consensus conclusions of the workshop "Software Infrastructure for Advanced Nuclear Physics Computing" (SANPC 24), which was held at Jefferson Lab on June 20-22, 2024. The workshop brought together members of the US Nuclear Physics community with data scientists and funding agency representatives, to discuss the challenges and opportunities in advanced computing for Nuclear Physics in the coming decade. Opportunities for sustainable support and growth are identified, within the context of existing and currently planned DOE and NSF programs.

==> Attendees.tex <==
\section{List of Workshop Attendees}\label{App:attendees}
% This is a list of SANPC attendees derived from
%   https://misportal.jlab.org/Ul/conferences/generic_conference/participants.cfm?conference_id=SANPC_2024
% It may be included as an appendix by adding (or uncommenting) '\input{Attendees}'
% line in Appendices.tex

\begin{longtable}{%
        l l }
\hline
{\bf Name} & {\bf Affiliation} \\
\hline
Adamson, Paul                            & National Nuclear Security Administration/NA-221  \\
Andreoli, Lorenzo                        & Old Dominion Univ./Thomas Jefferson National Laboratory \\
Arenas, Oscar                            & National Nuclear Security Administration/MSIIP  \\
Arratia, Miguel                          & Univ.\ of California, Riverside \\
Beyer, Kyle                              & Facility for Rare Isotope Beams, Michigan State Univ.  \\
Boehnlein, Amber                         & Thomas Jefferson National Laboratory \\
Britton, Thomas                          & Thomas Jefferson National Laboratory  \\
Brodsky, Jason                           & Lawrence Livermore National Laboratory \\
Brown, David                             & Brookhaven National Lab  \\
Bulgac, Aurel                            & Univ.\ of Washington \\
Carlson, Joseph                          & Los Alamos National Laboratory  \\
Chen, Jie                                & Thomas Jefferson National Laboratory \\
Chen, Yi                                 & Vanderbilt Univ.\  \\
Chung, Gyang                             & Department of Physics Virginia Tech \\
Cloet, Ian                               & Argonne National Laboratory  \\
Coleman, Stephen                         & RadiaSoft LLC \\
Cooper, Ren                              & Lawrence Berkeley National Laboratory  \\
Detmold, William                         & Massachusetts Institute of Technology \\
Detwiler, Jason                          & Univ.\ of Washington  \\
Diefenthaler, Markus                     & Thomas Jefferson National Laboratory \\
Dubey, Anshu                             & Argonne National Laboratory  \\
Edwards, Robert                          & Thomas Jefferson National Laboratory \\
Ehlers, Raymond                          & Univ.\ of California Berkeley/Lawrence Berkeley National Laboratory  \\
Flores, Abraham                          & Washington Univ.\ in St. Louis \\
Fossez, Kevin                            & Florida State Univ. \\
Gandolfi, Stefano                        & Los Alamos National Laboratory \\
Garland, Heather                         & Pacific Northwest National Laboratory  \\
Gavalian, Gagik                          & Thomas Jefferson National Laboratory \\
Gnech, Alex                              & Old Dominion Univ./Thomas Jefferson National Laboratory  \\
Godbey, Kyle                             & Facility for Rare Isotope Beams \\
Goodrich, Mike                           & Thomas Jefferson National Laboratory  \\
Guo, Xiaofeng                            & Department of Energy, SC-NP \\
Gysbers, Peter                           & Facility for Rare Isotope Beams  \\
Hansen, Ole                              & Thomas Jefferson National Laboratory \\
Hergert, Heiko                           & Facility for Rare Isotope Beams, Michigan State Univ.\  \\
Hix, William                             & Oak Ridge National Laboratory/Univ.\ of Tennessee \\
Jacobs, Peter                            & Lawrence Berkeley National Laboratory  \\
Jaiswal, Sunil                           & Ohio State Univ.\ \\
Jansen, Gustav                           & Oak Ridge National Laboratory  \\
Jeske, Torri                             & Thomas Jefferson National Laboratory \\
Jones, Florian                           & Lawrence Berkeley National Laboratory  \\
Kriesten, Brandon                        & Argonne National Laboratory \\
Kunnawalkam Elayavalli, Raghav           & Vanderbilt Univ.\  \\
Lancon, Eric                             & Brookhaven National Lab \\
Lawrence, David                          & Thomas Jefferson National Laboratory  \\
Lee, Dean                                & Michigan State Univ.\ \\
Liddick, Sean                            & Facility for Rare Isotope Beams/Michigan State Univ.  \\
Lin, Huey-Wen                            & Michigan State Univ. \\
Ma, Yuanzhuo                             & Michigan State Univ.  \\
Majumder, Abhijit                        & Wayne State Univ. \\
Manning, Andrew                          & NCSA, Univ.\ of Illinois Urbana-Champaign  \\
McGlynn, Patrick                         & Facility for Rare Isotope Beams \\
Melnitchouk, Wally                       & Thomas Jefferson National Laboratory  \\
Messer, Otis                             & Oak Ridge National Laboratory \\
Mestri, Siddhesh                         & Univ.\ of Mumbai  \\
Mihaila, Bogdan                          & National Science Foundation \\
Monahan, Chris                           & William \& Mary  \\
Monge Camacho, Henry                     & Oak Ridge National Laboratory \\
Morales Rosado, Romie                    & National Nuclear Security Administration/NA-22  \\
Munson, Todd                             & Argonne National Laboratory \\
Nachman, Ben                             & Lawrence Berkeley National Laboratory  \\
Nayak, Hemalata                          & William \& Mary \\
Nazarewicz, Witold                       & Michigan State Univ.  \\
Ng, Esmond                               & Lawrence Berkeley National Laboratory \\
O'Neal, Jared                            & Northwestern/Argonne National Laboratory  \\
Orginos, Kostas                          & William \& Mary/Thomas Jefferson National Laboratory \\
Panta, Anil                              & Thomas Jefferson National Laboratory  \\
Papenbrock, Thomas                       & Univ.\ of Tennessee/Oak Ridge National Laboratory \\
Paquet, Jean-Francois                    & Vanderbilt Univ.\  \\
Ploskon, Mateusz                         & Lawrence Berkeley National Laboratory \\
Potekhin, Maxim                          & Brookhaven National Lab  \\
Putschke, Joern                          & Wayne State Univ.\ \\
Ratti, Claudia                           & Univ.\ of Houston  \\
Ray, Adriel                              & Univ.\ of North Carolina Wilmington \\
Reed, Trevor                             & Florida International Univ. \\
Romero Alcalde, Eloy                     & Thomas Jefferson National Laboratory \\
Savage, Martin                           & Univ.\ of Washington  \\
Sawatzky, Brad                           & Thomas Jefferson National Laboratory \\
Schwiebert, Loren                        & Wayne State Univ.\  \\
Sen, Arindam                             & Ohio Univ.\ \\
Shahid, Muhammad                         & Georgia State Univ.\ \\
Shen, Chun                               & Wayne State Univ.\  \\
Soltz, Ron                               & Lawrence Livermore National Laboratory \\
Vujanovic, Gojko                         & Univ.\ of Regina  \\
Walker-Loud, Andre                       & Lawrence Berkeley National Laboratory \\
Wenaus, Torre                            & Brookhaven National Lab  \\
Yang, Liang                              & Univ.\ of California San Diego \\
Yapa, Nuwan                              & Florida State Univ.  \\
\hline
\end{longtable}


==> Makefile <==
DocName=SANPC
REV=NONE

TEXEXE=pdflatex -halt-on-error -file-line-error
#TEXEXE=xelatex

SHELL=/bin/bash

pdf: *.tex
	$(TEXEXE) $(DocName).tex
ifneq ("","$(wildcard *.bib)")  # untested as of yet...
	bibtex $(DocName)
#	biber --quiet --output-safechars   $(DocName)
endif
	$(TEXEXE) $(DocName).tex
	$(TEXEXE) $(DocName).tex

	@echo -e '\n\n                 ---------- WARNINGS ----------\n\n'
	grep Warning $(DocName).log | grep -v 'float specifier changed'
	@echo -e '\n\n                 ------------------------------\n\n'

diff:
ifeq ($(REV),NONE)
	@echo ''
	@echo 'Usage:  make REV=<git sha1>'
	@echo '    Use 'git log' and choose the commit you want to compare to.'
	@echo '    A new PDF will be generated with removals/addtions in red/blue.'
	@echo ''
else
	latexdiff-git --force --flatten --pdf -r $(REV) $(DocName).tex
endif

clean:
	rm -f $(DocName).{out,log,spl,bbl,blg,brf,lot,lof,toc} *.aux ${DocName}Notes.bib

realclean: clean
	rm -f $(DocName).pdf

